Active 3D Shape Reconstruction from Vision and Touch

Humans build 3D understandings of the world through active object exploration, using jointly their senses of vision and touch. However, in 3D shape reconstruction, most recent progress has relied on static datasets of limited sensory data such as RGB images, depth maps or haptic readings, leaving the active exploration of the shape largely unexplored. Inactive touch sensing for 3D reconstruction, the goal is to actively select the tactile readings that maximize the improvement in shape reconstruction accuracy. However, the development of deep learning-based active touch models is largely limited by the lack of frameworks for shape exploration. In this paper, we focus on this problem and introduce a system composed of: 1) a haptic simulator leveraging high spatial resolution vision-based tactile sensors for active touching of 3D objects; 2)a mesh-based 3D shape reconstruction model that relies on tactile or visuotactile signals; and 3) a set of data-driven solutions with either tactile or visuotactile priors to guide the shape exploration. Our framework enables the development of the first fully data-driven solutions to active touch on top of learned models for object understanding. Our experiments show the benefits of such solutions in the task of 3D shape understanding where our models consistently outperform natural baselines. We provide our framework as a tool to foster future research in this direction.

==> CheckList.tex <==
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope? \answerYes{ See the Sections 3, 4 and 5.}
  \item Did you describe the limitations of your work?
   \answerYes{See Section 6.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Section 6.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{We do not include theoretical results.}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{We do not include theoretical results.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{We provide detailed model description together with the hyper-parameters in supplementary material, and will release all code and trained models open source.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
     \answerYes{See Section 5 and the Supplemental Materials.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
   \answerYes{See Section 5, where standard deviation numbers are provided for all polices.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
   \answerYes{See the Supplemental Materials.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See Sections 3, 4, and 5 and the Supplemental Materials.}
  \item Did you mention the license of the assets?
    \answerYes{See the Supplemental Materials.}
  \item Did you include any new assets either in the supplemental material or as a URL?
   \answerNo{Our framework will be released upon publication.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{We use common 3D dataset that is widely used in computer vision.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
     \answerNo{We use common 3D dataset that is widely used in computer vision.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
   \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
   \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}




==> Setting.tex <==
In the following section, the active touch learning setting will be outlined. This will include detailed descriptions of how grasps are performed, the simulator in which touch signals are produced, the reconstruction method used to convert touch information from the environment to shape predictions, the dataset of 3D shape information used to train the reconstruction and active learning models, and the learning setting in which these models are trained


\subsection{Active touch simulator}
The goal of the proposed simulated tactile grasping environment is to perform and extract touch signals. A depiction of the steps in our active touch simulator is provided in Figure \ref{fig:grasping}. Conceptually, our simulator can be described in five steps. First, an object is loaded onto the environment (see point 1 in Figure \ref{fig:grasping}). An action space is defined around the 3D object by uniformly placing 50 points on a sphere centered at the center of the loaded object (see point 2 in Figure \ref{fig:grasping}). To choose a grasp, one of the points is selected and a 4 digit robot hand is placed such that its 3rd digit lies on the point and the hand's palm lies tangent to the sphere (see point 3 in Figure \ref{fig:grasping}). Then, the hand is moved towards the center of the object until it comes in contact with it (see point 4 in Figure \ref{fig:grasping}), and, finally, the fingers of the hand are closed until they reach the maximum joint angle, or are halted by the contact with the object (see point 5 in Figure \ref{fig:grasping}).

Each action is defined with its position on the sphere and is fully described by two angles. This parametriazation is selected specifically as it does not require any prior knowledge of the object, other then its center, and in simulation it consistently leads to successful interaction between the hand's touch sensors and the object's surface.

In our simulator, all steps are performed within a single python instance across the python robotics simulator PyBullet\cite{coumans2016pybullet}, the python rendering tool Pyrender \cite{pyrender}, and the PyTorch\cite{PyTorch}. For a given grasp and object, the object is loaded into PyBullet\cite{coumans2016pybullet}, along with a Wonik’s Allegro Hand \cite{Allegro} equipped with vision-based touch sensors \cite{Lambeta2020DIGIT} on each of its fingers, the point in space corresponding to the selected grasp is selected and the grasping procedure is performed as described in the above subsection using PyBullet's physics simulator. Pose information from the produced grasps is then extracted and used by Pyrender to render a depth map of the object from the perspective of each digit's sensors and a RGB image of the object from a fixed perspective. The depth maps are then converted into simulated touch signals \cite{V&T}. All steps in this procedure are performed in parallel or using GPU acccelered computing, and as a result across the 50 grasping options of 100 randomly chosen objects, simulated grasps and touch signals were produced in on average 0.0317 seconds each. Further details on this simulated environment are provided in the supplemental materials.


\begin{figure}
  \centering
  \includegraphics[width=1\textwidth]{Figures/current/grasping.pdf}
  \caption{A demonstration of each step in the grasping procedure. The object is loaded into the simulator, a sphere of possible action is imagined around it, an action is selected based on the current understanding of the object and the hand is placed on its corresponding point, the hand moves towards the center of the object, and a grasp is performed with touch signals extracted.}
  \label{fig:grasping}
\end{figure}


\subsection{Shape Reconstruction}
For 3D object reconstruction, we take inspiration from the chart-based reconstruction formulation of \cite{V&T} wherein shape is predicted by repeatedly deforming a collection of independent mesh surface elements (charts) using a graph convolutional network (GCN). Here, information from each touch signal is leveraged by predicting from it a single chart offline using a point cloud optimization, and the position of each chart is shared within the GCN while predicting global shape. The model can take as input either only touch signals, or a vision signal as well as touch signals. 
This 3D reconstruction method was altered in a number of ways to improve its accuracy and better suit our setting:
\begin{itemize}
\item Rather then using an inefficient offline point cloud optimization, we directly predict touch chart shape in mesh space using simple CNN which outputs positional updates to fixed initial chart. 
\item The formulation of the GCN and its training procedure was revised such that a variable number of touches signals can be passed to the same network.
\item Rather then pass vertex positions directly to the GCN, NERF positional embeddings \cite{NERF, SIREN} of them were passed to allow the network to capture higher frequency information.
\item Instead of using a single network for each iterative deformation, a unique network is used in the first pass to account the consistent input it must singularly account for.  
\end{itemize}
With these changes, the accuracy of predictions is demonstrated to be higher both with and without touch information, shape predicted from vision and touch can be performed with a pass through single pre-trained network, and variable number of touch signals can be expected. Further details with respect to the changes to this method can be found in Section \ref{} of the Appendix. The parameters of this reconstruction network are optimized to minimize the Chamfer Distance(CD) between the predicted and target surface \cite{Pix3D}. This distance function over surfaces is also chosen as the distance function which our active learning problem is defined. Further details with respect to the chamfer distance is provided in Section \ref{} of the Appendix. 


\subsection{Dataset of CAD models}
The dataset used for this project is made up of objects from 40000 objects sampled from the ABC dataset \cite{ABC, V&T}, a CAD model dataset of approximately one million objects. This dataset poses a much harder generalization challenge than other 3D object datasets, such as ShapeNet \cite{shapenet} due to its highly variable object shapes, and lack of clearly defined classes over which biases can be learned. The geometry of these objects were decimated such all object possess approximately 500 vertices. Those objects which could not be reduced to this size due to geometric constraints and those which possessed multiple disconnected parts were automatically removed, leading to set of 26545 usable object models.  This set of objects was split into 5 sets; 3 training sets of size 7700 object each, a validation set comprised 2000 objects, and a test set of size 1000. \footnote{Three training sets are leveraged, to mitigate the progressive overfitting which might occur from separately training networks which feed into one another on the same data.}


\subsection{Acquisition Settings}
We examine the performance of our models both for reconstruction and for active acquisitions across 4 learning settings:
\begin{itemize}
  \item V&T\_Poking: Vision and touch signals are leveraged, and in every grasp only the touch signal from the third digit of the hand is leveraged.
  \item T\_Poking: Only touch signals are leveraged, and in every grasp only the touch signal from the third digit of the hand is leveraged.
  \item V&T\_Grasping: Vision and touch signals are leveraged, and in every grasp the touch signals from each of the four digits are extracted. 
  \item T\_Grasping: Only touch signals are leveraged, and in every grasp the touch signals from each of the four digits are extracted. 
\end{itemize}

These setting represent learning how to touch an object in full daylight or in the dark(when using the vision signal and not), and by poking it or grasping it (when using a single finger or the full hand). 
